Minimizing Conjunctive Regular Path Queries

We study the minimization problem for Conjunctive Regular Path Queries (CRPQs) and unions of CRPQs (UCRPQs). This is the problem of checking, given a query and a number $k$, whether the query is equivalent to one of size at most $k$. For CRPQs we consider the size to be the number of atoms, and for UCRPQs the maximum number of atoms in a CRPQ therein, motivated by the fact that the number of atoms has a leading influence on the cost of query evaluation. We show that the minimization problem is decidable, both for CRPQs and UCRPQs. We provide a 2ExpSpace upper-bound for CRPQ minimization, based on a brute-force enumeration algorithm, and an ExpSpace lower-bound. For UCRPQs, we show that the problem is ExpSpace-complete, having thus the same complexity as the classical containment problem. The upper bound is obtained by defining and computing a notion of maximal under-approximation. Moreover, we show that for UCRPQs using the so-called "simple regular expressions" consisting of concatenations of expressions of the form $a^+$ or $a_1 + \dotsb + a_k$, the minimization problem becomes $\Pi^p_2$-complete, again matching the complexity of containment.

==> sec-minimization.tex <==

Here we define the main problems that we will study, namely the "minimization problem" for "CRPQs" and for "UCRPQs".


\AP
\decisionproblem{""Minimization problem"" for "CRPQs"}
{A finite alphabet $\A$, a "Boolean"  "CRPQ" $\gamma$ over $\A$ and $k \in \N$.}
{Does there exist a "CRPQ" $\delta$ over $\A$ with at most $k$ "atoms"\\ 
such that $\gamma \semequiv \delta$?}

\decisionproblem{\reintro{Minimization problem} for "UCRPQs"}
{A finite alphabet $\A$, a "Boolean"  "UCRPQ" $\Gamma$ over $\A$ and $k \in \N$.}
{Does there exist a "UCRPQ" $\Delta$ over $\A$ whose every "CRPQ" has at most $k$ "atoms" 
such that $\Gamma \semequiv \Delta$?}

%


\AP
We say that a (U)CRPQ is ""minimal"" if it is not equivalent to any (U)CRPQ having less maximum number of atoms.

\paragraph{On the chosen size measure}
  We observe that, as is the case for any minimization task, we have an implicit measure of `size', which in our case we have taken to be the maximum size of number of atoms.
  Why this choice?
  A na\"ive algorithm for the "evaluation" of a union of $t$ "CRPQs" with $k$-atoms on a graph database $G$ gives a rough bound of $O\big(t  k  (|\edges{G}|  r)^2 + t  |\vertex{G}|^{2k}\big)$ on a database with $n$ facts, where $r$ is the maximum size of the regular languages it contains, and $\edges{G}$, $\vertex{G}$ are the set of edges and vertices of $G$, respectively.\footnote{This is obtained by first materializing a table with the answers to each RPQ atom $x \atom{e} y$ of the query by listing all pairs of reachable vertices of $G$ in the synchronous product $G \times A_e$ between the database and the NFA $A_e$ for the regular expression $e$ in $O((|G|r)^2)$ ---and there are $tk$-many atoms---, and then evaluating each "CRPQ" as if it were a "conjunctive query" on the computed tables (each table having size at most $|\vertex{G}|^2$), in $O((|\vertex{G}|^2)^k) = O(|\vertex{G}|^{2k})$.}
  As we see, the most costly dependence is of $k$, since $G$ is the largest object ("ie", the database, several orders of magnitude larger than the remaining parameters in practice). The size of regular expressions and the number of unions have a less predominant multiplicative influence on the cost.
  Further, unions can be executed in parallel, which justifies the choice of taking the maximum size of the number of atoms of the CRPQ therein.
  However, other measures may also be reasonable. For example, taking the size to be the number of variables instead of the number of atoms as explored in \Cref{sec:varmin}.
  More complex measures including the size of regular expressions and the number of unions would need to take into account the drastically different roles of the parameters in the evaluation in view of the previous discussion ("eg", a simple sum of the parameters would not be a reasonable choice).
  %
  %





==> sec-removed.tex <==

\input{sec-treepatterns}  
\section{other things removed}
\paragraph{Strong Redundancy}
%
\paragraph{Completion}
%
\paragraph{Weak Redundancy}
%

A ""weak-homomorphism"" from a "CRPQ" $q$ to another "CRPQ" $q'$ is a mapping $h: \vars(q) \to \vars(q')$ such that for every atom $x \atom{L} y$ of $q$ there is a path $h(x) \atom{L_1} \dotsb \atom{L_n} h(y)$ from $h(x)$ to $h(y)$  in $q'$ where $L_1 \dotsb L_n \subseteq L$.
\begin{lemma}
  The "weak-homomorphism" relation is reflexive and transitive.
  If there is a "weak-homomorphism" from $q$ to $q'$, then $q' \contained q$.
\end{lemma}
An "atom" $\alpha$ of $q$ is ""weakly-redundant"" if there is a "weak-homomorphism" from $q$ to $q \setminus \set\alpha$.
%

=====================

Say that a class $\classCRPQ$ of CRPQs satisfies the \AP""uniform small model property""
if for every $\gamma \in \classCRPQ$, there exists a function
$\intro*\shrink{\gamma}\colon \Exp(\gamma) \times \N \to \Exp(\gamma)$ "st":
\begin{enumerate}
  \item for each $\gamma \in \classCRPQ$, for each $n \in \N$ and $\delta \in \classCRPQ$,
  if $\nbatoms{\delta} \leq n$ then for any $G \in \Exp(\gamma)$, $G \models \delta$ "iff"
  $\shrink{\gamma}(G, n) \models \delta$, and
  \item the size of $\shrink{\gamma}(G, n)$ only depends on $\gamma$ and $n$---but not $G$.
\end{enumerate} 
Note that $\shrink{\gamma}(G, n) \defeq G$ trivially satisfies the first point but not the second one.
In the name "uniform small model property" ``uniform'' refers to the fact
that the way we shrink $G$ onto $\shrink{\gamma}(G,n)$ is the same for all $\delta$---provided that $\nbatoms{\delta} \leq n$. The ``small model property'' part refers to the fact that to check if
$\gamma \contained \delta$, it suffices to check that all canonical databases of $\gamma$
of size at most $\nbatoms{\shrink{\gamma}(-, \nbatoms{\delta})}$ are models of $\delta$.

\begin{proposition}
  \AP\label{prop:containment-uniform-smp}
  If $\classCRPQ$ has the "uniform small model property", if $\gamma \in \classCRPQ$ and $\Delta$ 
  is a finite union of $\classCRPQ$-queries, then
  $\gamma \contained \Delta$ "iff" for every "canonical database" $G$ of $\gamma$,
  $\shrink{\gamma}(G, m) \models \Delta$
  where $m \defeq \max{\set{\nbatoms{\delta} \mid \delta \in \Delta}}$.
\end{proposition}

\begin{proof}
  The left-to-right implication is trivial. For the right-to-left implication, 
  let $G$ by any "canonical database" of $\gamma$,
  and assume by contradiction that $G \not\models \Delta$.
  Then for all $\delta \in \Delta$, $G \not\models \delta$,
  and so $\shrink{\gamma}(G, m) \not\models \delta$.
  It follows that $\shrink{\gamma}(G, m) \not\models \Delta$.
  Contradiction.
\end{proof}

\begin{proposition}
  \AP\label{prop:tree-patterns-uniform-smp}
  The class of tree patterns---and more generally CRPQs over $(a, a^+)$ or even over $(a, a^*)$---
  has the "uniform small model property", where $\shrink{\gamma}(G, n)$ consists
  in shrinking every "atom refinement" of size at least $n+1$ to an "atom refinement" of
  size $n$.
\end{proposition}

\begin{proof}
  TODO. Addref?
\end{proof}

\begin{corollary}
  \AP\label{coro:containment-union-tree-patterns-better}
  The containment problem of deciding if $\gamma \contained \Delta$, given:
  \begin{itemize}
    \item an integer $n$,
    \item a "tree pattern" $\gamma$ of size at most $n$,
    \item a union of "tree patterns" $\Delta$ "st" each $\delta \in \Delta$ has size at most $n$
    and deciding if a "tree pattern" $\delta$ belongs to $\Delta$ can be done in "NP" ("wrt" $n$),
  \end{itemize} 
  can be solved in "PiP2".
\end{corollary}

\begin{proof}
  By \Cref{prop:containment-uniform-smp,prop:tree-patterns-uniform-smp},
  $\gamma \contained \Delta$ "iff" for every "canonical database" $G$ of $\gamma$,
  there exists $\delta \in \Delta$ "st"
  $\shrink{\gamma}(G, n) \models \delta$.
  In turn, this is equivalent to asking that for every "canonical database" $G$ of $\gamma$
  of size at most $|\shrink{\gamma}(-, n)|$, then there exists $\delta\in \Delta$
  "st" $G \models \delta$.
  This concludes the proof that the problem lies in "PiP2" since by \Cref{prop:tree-patterns-uniform-smp}, $\nbatoms{\shrink{\gamma}(-, n)} = n^2$ so this
  upper bound is polynomial.
\end{proof}

\begin{proof}[Proof of \Cref{proof:union-tree-patterns}]
  \proofcase{Upper bound.}
  A "tree pattern" $\gamma$ is equivalent to a finite union of smaller "tree patterns"
  "iff" $\gamma \contained \App{\gamma}{\+C}{\textit{poly}}$ by \Cref{prop:max-under-approx},
  where $\+C$ is the class of all trees which are strictly smaller as "tree patterns"
  than $\gamma$.
  %
  But then %
  \[
    \App{\gamma}{\+C}{\textit{poly}} \semequiv 
    \{
      \alpha \in \CRPQ[\+C] \mid \exists \rho \in \Refin[\leq m](\gamma), 
      \rho \surjto \alpha
    \}.
  \]
  Each $\alpha$ has polynomial (in fact linear) size,
  and testing if $\alpha$ belongs to this latter union can be done in "NP" by definition,
  so \Cref{coro:containment-union-tree-patterns-better} provides an algorithm in "PiP2"
  for the problem.

  \proofcase{Lower bound.} %
\end{proof}

%

%
\input{sec-treelike}

\section{Removed from Discussion}
\subsection{Tree patterns} Tree pattern minimization on the class of tree patterns is "PiP2". Tree pattern minimization on the class of unions of tree patterns may be better. Possibly  the example of \cite[Fig.~9]{min-tree-patterns} is minimal, and yet it is equivalent to a union of small conjunctive queries.
Our results on "SRE" yield that unions of tree pattern minimization is still "PiP2", and hence that by going to a more expressive formalism we don't lose in complexity.

\begin{conjecture}
If a tree-like CRPQ is equivalent to a CRPQ of size $k$, then it is equivalent to a tree-like CRPQ of size $k$.
\end{conjecture}



\begin{open}
    What's the exact complexity of CRPQ (atom or variable) minimization?
\end{open}

\paragraph{Graphs with transitive edges} A very simple query language is the case of graphs with edges and transitive edges, which naturally corresponds to CRPQs having only two possible languages $a$ and $a^+$. In this simple case the upper bound for CRPQ minimality can be improved to XXX.

\begin{open}
    Does minimization of CRPQ on SRE have a better complexity than "2ExpSpace"?
\end{open}


==> sec-treelike.tex <==
\section{Tree-Like Queries}

%

\textcolor{Dark Ruby Red}{WARNING: In this section, all CRPQs are assumed to be positive, meaning
that no language can contain the empty word.}

\subsection{Forest-Shaped and DAG-Shaped Queries}

Say that a "CRPQ" is \AP""forest-shaped"" if its underlying directed multigraph 
is a directed simple forest---without self loops---, with the arrows going from roots to leaves.

We say that a CRPQ is \AP""semantically forest-shaped"" if it is
"semantically equivalent" to a CRPQ which is "forest-shaped".
A \AP""maximal canonical database"" of $\gamma$ is a "canonical database"
$G$ of $\gamma$ "st" for all "canonical database" $H$ of $\gamma$,
if $G \cohomto H$, then $H \cohomto G$.

Say that a CRPQ is \AP""DAG-shaped"" if its underlying directed multigraph
is a DAG---parallel edges are allowed, not self loops. If $\delta$ is "DAG-shaped",
define its \AP""unfolding"", denoted by \AP$\intro*\Unfold(\delta)$, as the following "CRPQ":
\begin{itemize}
	\item its variables are exactly labelled path of $\delta$
	of the form $x_0 \atom{L_1} \cdots \atom{L_n} x_n$ with $n\in \N$
	and $x_0$ is a vertex of $\delta$ with no predecessor;
	\item the atoms exactly go from $x_0 \atom{L_1} \cdots \atom{L_n} x_n$
	to $x_0 \atom{L_1} \cdots \atom{L_n} x_n \atom{L_{n+1}} x_{n+1}$,
	with label~$L_{n+1}$.
\end{itemize}

\begin{fact}
	\AP\label{fact:unfolding-is-forest}
	If $\delta$ is a "DAG-shaped CRPQ", then $\Unfold(\delta)$ is a "forest-shaped CRPQ",
	and moreover $\delta \contained \Unfold(\delta)$.
\end{fact}

The rest of this section is devoted to proving the following result.

\begin{theorem}
	\AP\label{thm:charac-semantically-forest-shaped}
	Let $\delta$ be a "CRPQ". The following are equivalent:
	\begin{enumerate}
		\item $\delta$ is "semantically forest-shaped",
		\item $\delta$ is "DAG-shaped" and
			for all "maximal canonical database" $D$ of $\delta$, the "core" of $D$ is a forest,
		\item $\delta$ is "DAG-shaped" and $\delta \semequiv \Unfold(\delta)$. 
	\end{enumerate}
\end{theorem}

Note that since "semantical equivalence" is decidable in "ExpSpace" and
since $\Unfold(\delta)$ has exponential size, it follows that one can test if
a "CRPQ" is "semantically forest-shaped" in "2ExpSpace".

\subsection{Semantically DAG-Shaped Queries}

\begin{proposition}
	A "CRPQ" is "semantically DAG-shaped" "iff" it is "DAG-shaped".
\end{proposition}

\begin{proof}
todo
\end{proof}

\begin{corollary}
	\AP\label{coro:sem-forest-implies-DAG}
	If a "CRPQ" is "semantically forest-shaped", then it is "DAG-shaped".
\end{corollary}

\subsection{Semantically Forest-Shaped}

From the fact that a "CRPQ" $\delta$ is equivalent to a "forest-shaped" query $\phi$
we know that for all "canonical database" $D_0$ of $\delta$, since $\delta \contained \phi$,
there exists a "canonical database" $F_0$ of $\phi$ "st" $D_0 \cohomto F_0$.
But dually since $\phi \contained \delta$, there exists $D_1 \cdb \delta$ "st" $F_0 \cohomto D_1$.
By induction---and the axiom of choice---we obtain an infinite co-chain of "homomorphisms"
\[
	D_0 \cohomto F_0 \cohomto D_1 \cohomto F_1 \cohomto \cdots \cohomto D_n \cohomto F_n \cohomto \cdots.
\]
We show that co-chains of forests are actually quite simple.

\begin{fact}
	If $F_0 \cohomto F_1 \cohomto \cdots \cohomto F_n \cohomto \cdots$
	is an infinite co-chain of "homomorphisms" betweens "forests", 
	then there exists $n \in \N$ "st" all $F_m$ with $m\geq n$
	are "hom-equivalent" to one another.
\end{fact}

\begin{proof}
	For all $n \in \N$, from $F_n \cohomto F_{n+1}$ it follows that
	the maximal depth of a tree in $F_{n+1}$ is smaller or equal to the
	maximal depth of a tree in $F_{n}$. So, at some point this parameter
	must become stationary, say $d$. Then observe that there
	are finitely many forests with depth at most $d$, up to "hom-equivalence",
	and hence, one of these must occur infinitely often in the co-chain.
\end{proof}

\begin{corollary}
	\AP\label{coro:all-cdb-are-dominated-by-forests}
	If $\delta$ is "semantically forest-shaped", then for any
	$D \cdb \delta$, there exists $D' \cdb \delta$ such that
	$D \cohomto D'$, $D'$ is "maximal" and the core of $D'$ is a forest.
\end{corollary}

We can now proceed with the proof of \Cref{thm:charac-semantically-forest-shaped}, after giving a
proposition that will prove useful.

\begin{proposition}
	\AP\label{prop:hom-from-forest}
	Let $F$ be a forest and $D$ a graph. If $F \homto D$ then $F \homto \Unfold(D)$.
\end{proposition}

\begin{proof}
	The "homomorphism" $F \homto \Unfold(D)$ can be defined by induction on $F$, from roots
	to leaves.
\end{proof}

\begin{proof}[Proof of \Cref{thm:charac-semantically-forest-shaped}.]
	\proofcase{$(1) \Rightarrow (2)$.} This follows from
	\Cref{coro:sem-forest-implies-DAG,coro:all-cdb-are-dominated-by-forests}.

	\proofcase{$(2) \Rightarrow (3)$.} By \Cref{fact:unfolding-is-forest} we have $\delta \contained \Unfold(\delta)$ so it suffices to prove the converse "containment".
	Let $U$ be a "canonical database" of $\Unfold(\delta)$. Then there exists $D \cdb \delta$
	"st" $U = \Unfold(D)$. By \Cref{coro:all-cdb-are-dominated-by-forests} there exists
	$D' \cdb \delta$ "st" $D \cohomto D'$ and the core of $D'$ is a forest. So $D \cohomto \core(D')$, and so by \Cref{prop:hom-from-forest}, since $\core(D')$ is a "forest",
	then $\Unfold(D) \cohomto \core(D')$ "ie" $\Unfold(D) \cohomto D'$, which proves
	that $\Unfold(D) \models \delta$. Therefore, $\Unfold(\delta) \contained \delta$.

	\proofcase{$(3) \Rightarrow (1)$.} This is because $\Unfold(\delta)$ is "forest-shaped"
		by \Cref{fact:unfolding-is-forest}.
\end{proof}


==> sec-treepatterns.tex <==
\section{Not included: Tree-like Queries}

%
The minimization of ""tree patterns"" has been thoroughly studied \cite{min-tree-patterns}. 
A "tree pattern" can be seen in our context as a special kind of tree-like "CRPQ". Let us call a \AP""pseudo-tree"" to any directed multigraph such that (i) it has no parallel edges (in particular no parallel self-loops) and (ii) once the self-loops are removed, it is a directed `root-to-leaves' tree.
Let us fix an alphabet letter $e \in \A$ which will be used to model the child relation.
A \AP""tree pattern CRPQ"" is then any "CRPQ" such that
\begin{itemize}
  \item the underlying directed multigraph of the query is a "pseudo-tree"; and
  \item its "self-loops" are of the form $x \atom{a} x$ for some $a \in \A \setminus \set{e}$
  \item its remaining "atoms" are form (a) $x \atom{e^+} y$ or (b) $x \atom{e} y$.
\end{itemize}
A \AP""pseudo-tree database"" is a "graph database" such that
\begin{itemize}
  \item the underlying directed multigraph of the query is a "pseudo-tree"; and
  \item every "vertex" $v$ there is an edge $(v,a,v)$ for some $a \in \A \setminus \set{e}$
  \item its remaining "edges" are of the form $(v,e,v')$.
\end{itemize}

\knowledgenewrobustcmd{\treePatEnc}[1]{\cmdkl{\textup{\bf t}_{#1}}}
We can then define a bijection between "tree pattern CRPQs" and "tree patterns". Given a "tree pattern CRPQ" $q$, we define $\intro*\treePatEnc{q}$ to be the "tree pattern" consisting of treating self-loops as node labels, $x \atom{e^+} y$ as the descendant relation, and $x \atom{e} y$ as the child relation. It is easy to see that $\set{q \mapsto \treePatEnc{q}}$ is a bijection. 

\begin{lemma}\AP\label{lem:treepat-crpq}
  A "tree pattern CRPQ" $q$ is "atom-minimal" if, and only if, $\treePatEnc{q}$ is minimal (among tree patterns over trees).
\end{lemma}
\begin{proof}
  \proofcase{Left-to-right.}
  Observe the following:
  \begin{claim}\AP\label{cl:atommin-over-trees=treepatmin}
    The following are equivalent for each "tree pattern CRPQ" $q$:
    \begin{enumerate}
      \item $q$ is "atom-minimal" among "tree pattern CRPQs" over "pseudo-tree databases";
      \item $\treePatEnc{q}$ is minimal among "tree patterns" over trees.
    \end{enumerate}  
  \end{claim}
  \begin{claim}\AP\label{cl:equiv-overtrees-overgraphs}
    Two "tree pattern CRPQs" are "equivalent" over "pseudo-tree databases" if, and only if, they are "equivalent" over arbitrary "graph databases".
  \end{claim}
  In view of \Cref{cl:atommin-over-trees=treepatmin,cl:equiv-overtrees-overgraphs} we have that
    if a "tree pattern CRPQ" $q$ is "atom-minimal" (among all "CRPQs" over arbitrary "graph databases"), then $\treePatEnc{q}$ is "minimal" (among "tree patterns" over trees).

  \proofcase{Right-to-left.}
  By \Cref{cl:atommin-over-trees=treepatmin,cl:equiv-overtrees-overgraphs}, it suffices to show that if a "tree pattern CRPQ" is "atom-minimal" among "tree pattern CRPQs", then it is also "atom-minimal" among all "CRPQs". In other words, if a "tree pattern CRPQs" $q$ is "equivalent" to a "CRPQ" $q'$ with fewer "atoms", then it is also equivalent to a "tree pattern CRPQ" $q''$ with fewer "atoms".
  %
\end{proof}

As a consequence of \cite[Theorem~3.1]{min-tree-patterns} and the previous \Cref{lem:treepat-crpq} we then have:
\begin{corollary}
  The "atom-minimization problem" for "tree pattern CRPQs" is "SigmaP2"-complete.
\end{corollary}

